Beyond Data Samples: Aligning Differential Networks Estimation with Scientific Knowledge

Learning the differential statistical dependency network between two contexts is essential for many real-life applications, mostly in the high dimensional low sample regime. In this paper, we propose a novel differential network estimator that allows integrating various sources of knowledge beyond data samples. The proposed estimator is scalable to a large number of variables and achieves a sharp asymptotic convergence rate. Empirical experiments on extensive simulated data and four real-world applications (one on neuroimaging and three from functional genomics) show that our approach achieves improved differential network estimation and provides better supports to downstream tasks like classification. Our results highlight significant benefits of integrating group, spatial and anatomic knowledge during differential genetic network identification and brain connectome change discovery.

==> 020-backDiffShort.tex <==
\subsection{Basics and $\Delta$ as differential GGM }
\label{sec:back}

Estimating differential GGMs includes two sets of observed samples, denoted as two matrices $\Xb_{c} \in \RR^{n_{c} \times p}$ and  $\Xb_{d} \in \RR^{n_{d} \times p}$. $\Xb_{c}$ and $\Xb_{d}$ assume i.i.d drawn from two normal distributions $N_p(\mu_c, \Sigma_c)$ and $N_p(\mu_d, \Sigma_d)$ respectively. Here $\mu_c, \mu_d \in \RR^{p}$ describe the mean vectors and  $\Sigma_c,\Sigma_d \in \RR^{p \times p}$ represent covariance matrices. The goal of differential GGMs is to estimate the structural change $\Delta$ defined by \cite{zhao2014direct} \footnote{For instance, on data samples from a controlled drug study, `c' may represent the `control' group and `d' may represent the `drug-treating' group. Using which of the two sample sets as `c' set (or `d' set) does not affect the computational cost and does not influence the statistical convergence rates.}. 
\begin{equation}
\label{def:diffNet}
\Delta = \Omega_{d} - \Omega_{c}
\end{equation}
Here  $\Omega_c := (\Sigma_c)^{-1}$ and $\Omega_d := (\Sigma_d)^{-1}$ are two precision matrices. The sparsity pattern of the precision matrix of a GGM encodes the conditional dependency  structure of the GGM. This means, $\Delta$ describes how the magnitude of conditional dependency differs between two conditions. 
A sparse $\Delta$ means few of its entries are non-zero, indicating a differential network with few edges.  However, when in high-dimensional regimes, $\mathcal{B}(\hat{\Sigma}_d, \hat{\Sigma}_c)$ is not well-defined because $\hat{\Sigma}_c$ and $\hat{\Sigma}_d$ are rank-deficient (thus not invertible). %
\footnote{$\mathcal{B}$ refers to Backward Mapping, and $\mathcal{B}^*$ denotes proxy backward mapping.}

==> 026-relateDiff.tex <==

\subsection{Connecting to other Differential Graphical Models:} 
 \label{sec:diffrel}

Undirected Graphical models (UGM) have been popular tools for estimating variable dependencies from observed multivariate samples. Two classes of UGM have gained significant attention in the literature: (1) Gaussian Graphical Models (GGMs) and extensions like nonparanormal UGMs model continuous inputs, and (2) Ising models are for categorical variables. We focus on GGMs here.

Recent literature on differential GGMs fall into four kinds.  (1) \textbf{Multitask MLE based}. Multiple studies \citep{zhang2012learning,danaher2013joint,honorio2010multi} used the fused norm or similar to learn the differential network via multi-tasking and followed the regularized maximum likelihood estimation (MLE) formulation. However, in a setting with large number of variables, the strategy needs to assume each dependency structure is sparse and has been found to produce many spurious differences \citep{de2010differential}. (2) \textbf{Density ratio based:}. Recently, \cite{liu2017learning,liu2014direct} used density ratio estimation (SDRE) to directly learn structural difference without having to identify the dependency structure of each. (3) \textbf{Constrained $\ell_1$ minimization based}. Diff-CLIME, another regularized convex program, was proposed to directly learn structural changes without going through the learning of each GGM ~\citep{zhao2014direct}. (4) \textbf{Elementary estimator based}. The last category extends a so-called Elementary Estimator (EE) \citep{yang2014elementary1,yang2014elementary,yang2014elementary2} for direct learning of differential GGM. The resulting  estimator, {\diffee} \citep{wang2017fastchange}, is solved through a faster and closed-form solution, allowing it to scale to a large number of variables. We review these methods in more detail (with equations) in Section~\ref{sec:rel}.  


\methodName designs a new hybrid norm and provides flexibility to enforce many different kinds of structure priors including like group sparsity, hub structure, or combinations. The {\diffee} estimator is a special case of \methodName.  

==> 0315-shortBayesian.tex <==
\paragraph{Bayesian Interpretation: \hspace{2mm}}

We can interpret the additional edge-level knowledge via a hierarchical Bayesian interpretation.
Essentially, we assume the $\{i,j\}$-th entry of $\Delta$ follows a Laplace distribution:
\begin{equation}
P(\Delta_{i,j}|W_{i,j}, \sigma) \sim \dfrac{W_{i,j}}{\sigma}exp(-\dfrac{W_{i,j}\times |\Delta_{i,j}|}{\sigma})
\label{eq:bayesian}
\end{equation}

When $W_{i,j}$ is larger, $P(\Delta_{i,j}|W_{i,j}, \sigma)$ tends to concentrate on 0. Similarly, the group evidence corresponds to a scale mixture of normals \citep{kyung2010penalized}.









==> 041-ExpSim-Short.tex <==
\section{Experiment 1: Simulation Datasets}

==> 043-ExpSimSettingsShort.tex <==
{\bf Experiment Design}: We consider three different types of known edge knowledge $W_E$ generated from the spatial distance and groups to simulate related anatomical regions. These three are distinguished by different $p=\{116,160,246\}$.  We vary  $n_c$ and $n_d$ in $\{p/2,p/4,p,2p\}$ to account for both high dimensional and low dimensional cases. The sparsity of the underlying differential graph is controlled by $s=\{0.125,0.25,0.375,0.5\}$ and $s_G$. This results in $126$ different datasets representing diverse settings: multiple $p$, number of samples $n_c$ and $n_d$,  sparsity $s$ and number of groups $s_G$ and three data settings. 

==> 045-Table.tex <==
\begin{table*}[htb]
\centering
\scriptsize
\begin{tabular}{r|r|r|r|r|r|r}\toprule
\multirow{2}{*}{Method} & \multicolumn{1}{c|}{Data-EG(Time)} &
      \multicolumn{3}{c|}{Data-EG(F1-Score)} &
      \multicolumn{1}{c|}{Data-G(Time)} & \multicolumn{1}{c}{Data-G(F1-Score)} \\
       \cmidrule(r){2-7}
  		
          &  W2($p=246$)      & W1($p=116$)     &   W2($p=246$)   & W3($p=160$)     & W2($p=246$)    & W2($p=246$)     \\\midrule
KDiffNet-EG & 3.270$\pm$0.182 & \bf{0.704}$\pm$0.022  & \bf{0.926}$\pm$0.001 & \bf{0.934}$\pm$0.002 & * &    * \\\hline
KDiffNet-G & 0.006$\pm$0.00 & 0.578$\pm$0.001 & 0.565$\pm$0.00 & 0.576$\pm$0.00 &   0.006$\pm$0.000 &    {\bf 0.860$\pm$0.000}   \\\hline
KDiffNet-E & 0.005$\pm$0.001 & 0.686$\pm$0.024 & 0.918$\pm$0.001 & 0.916$\pm$0.002 & * & *  \\\hline\midrule		
JEEK \cite{wang2017fast}     &  10.476$\pm$0.054   & 0.571$\pm$0.010 & 0.582$\pm$0.001 & 0.582$\pm$0.001 & * & *       \\\hline		
NAK\cite{bu2017integrating}       &   6.520$\pm$0.184 & 0.225$\pm$0.013 & 0.198$\pm$0.011 & 0.203$\pm$0.005 &     *   &    *      \\ \hline \midrule		
SDRE\cite{liu2014direct}     &   28.807$\pm$1.673 & 0.573$\pm$0.11 & 0.568$\pm$0.006 & 0.574$\pm$0.11 &    11.764$\pm$1.23 &   0.318$\pm$0.10     \\\hline 		
DIFFEE\cite{wang2017fastchange}    &   0.005$\pm$0.00   & 0.570$\pm$0.001 & 0.562$\pm$0.00 & 0.570$\pm$0.00 & 0.004$\pm$0.000 & 0.131$\pm$0.131  \\\hline		
JGLFUSED\cite{danaher2013joint}   &   109.15$\pm$13.659  & 0.512$\pm$0.001 & 0.489$\pm$0.001 & 0.504$\pm$0.001 &   112.441$\pm$6.362 &  0.060$\pm$0.00\\\hline
Number of Datasets   & 14    & 14 & 14 &  14 & 14   &  14\\\hline
\bottomrule

\end{tabular}
\caption{\footnotesize Mean Performance(F1-Score)  and Computation Time(seconds) with standard deviation for $10$ random seeds given in parentheses of \methodNameEV, \methodNameE, \methodNameV and baselines for  simulated data. We evaluate over $126$ datasets: $14$ variations in each of the three spatial matrices $W_E$: $p=116$(W1), $p=246$(W2),  and $p=160$(W3)  for the three data settings: Data-EG, Data-E and Data-G. $*$ indicates not applicable.}
\label{tab:summary}
\end{table*}




==> 046-dl-connect.tex <==
\subsection{Comparing with deep learning based structure discovery}

